Idealize - A Notion of Idea Strength

Business Entrepreneurs frequently thrive on looking for ways to test business ideas, without giving too much information. Recent techniques in startup development promote the use of surveys to measure the potential client's interest. In this preliminary report, we describe the concept behind Idealize, a Shiny R application to measure the local trend strength of a potential idea. Additionally, the system might provide a relative distance to the capital city of the country. The tests were made for the United States of America, i.e., made available regarding native English language. This report shows some of the tests results with this system.

==> images/data/graph_inesc.tex <==

\pgfplotstableread[col sep=semicolon]{images/data/results_Inesc_elapsed_time.txt}\dataTableElapsedTime
\pgfplotstableread[col sep=semicolon]{images/data/results_Inesc_cum_time.txt}\dataTableCumulativeTime
\pgfplotstableread[col sep=semicolon]{images/data/results_Inesc_speedup.txt}\dataTableSpeedup


% Preamble: \pgfplotsset{width=7cm,compat=smooth,mark=*,red,mark size=0.75,mark size=0.53}
\pgfplotsset{footnotesize}
\begin{center}% note that \centering uses less vspace...
\begin{tikzpicture}[scale=0.8]
\begin{axis}[
title={Speedup Ratio},
%ylabel = nodes,
%ymode=log,
%ymax = 5000,
%ymin = 1000,
xticklabels={,,},
%yticklabel style={text width=0.5cm},
%width=5cm,
%height=3cm
legend style={draw=none}
]
%\addplot[smooth,mark=square,red!50,mark size=0.75] table[y = speedup] from \dataTableSpeedup;
%\addplot[dashed,mark=triangle,blue!50,mark size=0.75] table[y = speedupinc] from \dataTableSpeedup;

\addplot[smooth,mark=square,blue,mark size=1] table[y = speedup] from \dataTableSpeedup;

\end{axis}
\end{tikzpicture}
%
\begin{tikzpicture}[scale=0.8]
\begin{axis}[
title={\qquad Elapsed Time (s)},
%ymode=log,
%ymax = 50000,
%ymin = 100,
%yticklabels={,,},
xticklabels={,,},
%width=5cm,
%height=3cm
]
%\addplot[smooth,mark=o,green,mark size=0.75] table[y = batch] from \dataTableElapsedTime;
%\addplot[smooth,mark=square,red,mark size=0.75] table[y = Window-based] from \dataTableElapsedTime;
%\addplot[dashed,mark=triangle,blue,mark size=0.75] table[y = Inc] from \dataTableElapsedTime;

\addplot[smooth,mark=o,red,mark size=1] table[y = batch] from \dataTableElapsedTime;
\addplot[smooth,mark=square,blue,mark size=1] table[y = IS-TFIDF & ICS ] from \dataTableElapsedTime;

\end{axis}
\end{tikzpicture}
%
\begin{tikzpicture}[scale=0.8]
\begin{axis}[
legend columns=-1,
legend entries={Batch, IS-TFIDF \& ICS},
%legend entries={TextRank, Window-based (Streaming TextRank), incremental (incremental TextRank)},
%legend style={font=\tiny},
legend to name=named,
title={\qquad Cumulative Time (s)},
%ymode=log,
%ymax = 50000,
%ymin = 100,
%yticklabels={,,},
xticklabels={,,},
%width=5cm,
%height=3cm
]
%\addplot[smooth,mark=o,green,mark size=0.75] table[y = batch] from \dataTableCumulativeTime;
%\addplot[smooth,mark=square,red,mark size=0.75] table[y = Window-based] from \dataTableCumulativeTime;
%\addplot[dashed,mark=triangle,blue,mark size=0.75] table[y = Inc] from \dataTableCumulativeTime;

\addplot[smooth,mark=o,red,mark size=1] table[y = batch] from \dataTableCumulativeTime;
\addplot[smooth,mark=square,blue,mark size=1] table[y = IS-TFIDF & ICS] from \dataTableCumulativeTime;

\end{axis}
\end{tikzpicture}
\\
\ref{named}
\end{center}


==> images/data/graph_reuters.tex <==

\pgfplotstableread[col sep=semicolon]{images/data/results_Reuters_elapsed_time.txt}\dataTableElapsedTime
\pgfplotstableread[col sep=semicolon]{images/data/results_Reuters_cum_time.txt}\dataTableCumulativeTime
\pgfplotstableread[col sep=semicolon]{images/data/results_Reuters_speedup.txt}\dataTableSpeedup


% Preamble: \pgfplotsset{width=7cm,compat=smooth,mark=*,red,mark size=0.75,mark size=0.53}
\pgfplotsset{footnotesize}
\begin{center}% note that \centering uses less vspace...
%
% Nodes
%

\begin{tikzpicture}[scale=0.8]
\begin{axis}[
title={Speedup Ratio},
%ylabel = nodes,
%ymode=log,
%ymax = 5000,
%ymin = 1000,
xticklabels={,,},
%yticklabel style={text width=0.5cm},
%width=5cm,
%height=3cm
legend style={draw=none}
]
%\addplot[smooth,mark=square,red!50,mark size=0.75] table[y = speedup] from \dataTableSpeedup;
%\addplot[dashed,mark=triangle,blue!50,mark size=0.75] table[y = speedupinc] from \dataTableSpeedup;

\addplot[smooth,mark=square,blue,mark size=1] table[y = speedup] from \dataTableSpeedup;

\end{axis}
\end{tikzpicture}
%
\begin{tikzpicture}[scale=0.8]
\begin{axis}[
title={\qquad Elapsed Time (s)},
%ymode=log,
%ymax = 50000,
%ymin = 100,
%yticklabels={,,},
xticklabels={,,},
%width=5cm,
%height=3cm
]
%\addplot[smooth,mark=o,green,mark size=0.75] table[y = batch] from \dataTableElapsedTime;
%\addplot[smooth,mark=square,red,mark size=0.75] table[y = Window-based] from \dataTableElapsedTime;
%\addplot[dashed,mark=triangle,blue,mark size=0.75] table[y = Inc] from \dataTableElapsedTime;

\addplot[smooth,mark=o,red,mark size=1] table[y = batch] from \dataTableElapsedTime;
\addplot[smooth,mark=square,blue,mark size=1] table[y = IS-TFIDF & ICS] from \dataTableElapsedTime;

\end{axis}
\end{tikzpicture}
%
\begin{tikzpicture}[scale=0.8]
\begin{axis}[
legend columns=-1,
legend entries={Batch, IS-TFIDF \& ICS},
%legend entries={TextRank, Window-based (Streaming TextRank), incremental (incremental TextRank)},
%legend style={font=\tiny},
legend to name=named,
title={\qquad Cumulative Time (s)},
%ymode=log,
%ymax = 50000,
%ymin = 100,
%yticklabels={,,},
xticklabels={,,},
%width=5cm,
%height=3cm
]
%\addplot[smooth,mark=o,green,mark size=0.75] table[y = batch] from \dataTableCumulativeTime;
%\addplot[smooth,mark=square,red,mark size=0.75] table[y = Window-based] from \dataTableCumulativeTime;
%\addplot[dashed,mark=triangle,blue,mark size=0.75] table[y = Inc] from \dataTableCumulativeTime;

\addplot[smooth,mark=o,red,mark size=1] table[y = batch] from \dataTableCumulativeTime;
\addplot[smooth,mark=square,blue,mark size=1] table[y = IS-TFIDF & ICS] from \dataTableCumulativeTime;

\end{axis}
\end{tikzpicture}
\\
\ref{named}
\end{center}

